Cohomological Obstructions for Mittag-Leffler Problems

This is an extensive survey of the techniques used to formulate generalizations of the Mittag-Leffler Theorem from complex analysis. With the techniques of the theory of differential forms, sheaves and cohomology, we are able to define the notion of a Mittag-Leffler Problem on a Riemann surface as a problem of passage of data from local to global, and discuss characterizations of contexts where these problems have solutions.

==> esquisse.tex <==
%Parte I Preliminares
%% fibrados vetoriais em variedades suaves --> bott-tu, escolha de exemplos do borges-tengan II
%% (co)homologia singular (??) --> rotman, bott-tu
%% Superficies de Riemann e funcoes meromorfas
%% O Problema de Mittag-Leffler no plano


%Parte II Cohomologia
%% Formas diferenciais e cohomologia de De Rham
%% Formas diferenciais em superficies de Riemann (em variedades complexas?)
%% Cohomologia de Dolbeault
%% Cohomologia de Cech
%% Feixes
%% Formulacao Cohomologica do Problema de Mittag-Leffler

%Apendices
%% x Integracao de formas/Analise/Geometria? acho q n (isso vai estar, a priori, no texto)
%% Sobre as provas da Dualidade de Serre e Riemann-Roch e teorema de leray(isso vai estar no texto na secao da formulacao cohomologica do problema de ml)
%% (Aneis locais noetherianos,) DVRs e divisores & fibrados de linha? acho q n tb (na vdd isso e importante, vou comecar as aplicacoes com isso - divisores e fibrados de linha/feixes inversiveis e hirzerbruch riemann roch)
%% Teoremas de Mergulho e Algebrizacao: GAGA, Chow e Kodaira --> GAGA
%% Sequencias espectrais (isso vai estar, a priori, no texto)
%% Mittag-Leffler & Bourbaki
%% Cohomological formulation of the First Cousin Problem on manifolds of arbitrary dimension (gunning rossi p 248 har ex 1.21)

%apendices atualiado
%%riemann roch and possibly serre duality will be in the gaga section most likely, together with divisors and line bundles and hrr: the idea is to most likely follow sections one and three of chap 1 of griffiths harris, and then talk about gaga

%% spectral sequences, following dfat and vakil

%%mittag-leffler and bourbaki

%quotes

%% miles davis: if you understood everything i said, you'd be me!
%% riemanns apology for his theory of surfaces
%% serres letter to grothendieck on his effort to get used to cohomological language
%% grothendieck on inertia and stubborness in the beginning of PS

%%The idea behind this document is to tie together some of my background in things that I have studied during my undergraduate years, in commutative algebra, algebraic geometry, complex analysis, as well as algebraic topology and category theory. My motivation was to extend my knowledge to a point where they all meet, by searching for interesting relations among them.
